Models, Methods and Network Topology: Experimental Design for the Study of Interference

How should a network experiment be designed to achieve high statistical power? Ex- perimental treatments on networks may spread. Randomizing assignment of treatment to nodes enhances learning about the counterfactual causal effects of a social network experiment and also requires new methodology (ex. Aronow and Samii 2017a; Bow- ers et al. 2013; Toulis and Kao 2013). In this paper we show that the way in which a treatment propagates across a social network affects the statistical power of an ex- perimental design. As such, prior information regarding treatment propagation should be incorporated into the experimental design. Our findings justify reconsideration of standard practice in circumstances where units are presumed to be independent even in simple experiments: information about treatment effects is not maximized when we assign half the units to treatment and half to control. We also present an exam- ple in which statistical power depends on the extent to which the network degree of nodes is correlated with treatment assignment probability. We recommend that re- searchers think carefully about the underlying treatment propagation model motivat- ing their study in designing an experiment on a network.

==> toyExample.tex <==


% latex table generated in R 3.4.3 by xtable 1.8-2 package
% Wed Jan 17 08:47:36 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrr}
  \hline
 & A & B & C & D & E & F \\ 
  \hline
A & 0 & 1 & 1 & 0 & 0 & 0 \\ 
  B & 1 & 0 & 0 & 0 & 0 & 0 \\ 
  C & 1 & 0 & 0 & 0 & 0 & 1 \\ 
  D & 0 & 0 & 0 & 0 & 1 & 0 \\ 
  E & 0 & 0 & 0 & 1 & 0 & 0 \\ 
  F & 0 & 0 & 1 & 0 & 0 & 0 \\ 
   \hline
\end{tabular}
\caption{Adjacency matrix of a simple 6 node network with 4 edges.} 
\label{fig:toy-example-adj}
\end{table}To motivate this discussion, and introduce the primary statistical method, we introduce a toy example using a simpler model and test statistic than will be later employed. The primary goal of this toy example is demonstrate how the \emph{power}, the probability of rejecting a false null hypothesis, of the statistical approach can depend heavily on the treatment assignment mechanism, the network, and the interaction of these two features in generating the observed outcome. Table~\ref{fig:toy-example-adj} shows the adjacency matrix of this simple network. We label this network $S$. 
Additionally, for each node we have a background covariate $\bx = (2.4,0.6,2.2,0.9,0.4,0)'$. The covariate and the network combine with the treatment assignment $\bZ$ in two outcome models:
\begin{align}
  \bY(\bZ) &= \bx + \theta \bZ \label{eq:toy-no-spill} \\ 
  \bY(\bZ) &= \bx + \theta \bZ + (1 - \bZ) \theta I(S \bZ > 0) \label{eq:toy-no-spill2}
\end{align}
In the first model, as each node's outcome depends only on its own treatment status, this model involves no spillover. The second model, on the other hand, treated units share their benefit with any untreated neighbors. 
For simplicity, we fix the true $\theta$ at 1 in both models. To constrast different assignment mechanisms, we consider two treatment assignment mechanisms: assign two units to treatment, four to control (``unbalanced''); three units to treatment, three to control (``balanced''). For each possible treatment strategy, we can enumerate all possible treatment allocation (15 for the unbalanced case and 20 for the balanced case). For each allocation, we can generate the $\bY$ that would be observed if $\theta = 1$. For each of these observed $\bY$, we then apply the randomization inference procedure, using a squared t-statistic, to compute $p$-values for the (false) hypothesis that treatment had no effect (i.e., $\theta = 0$). This results in a $p$-value that would be observed for each possible randomization. For a given $\alpha$-level, the randomization method that has more $p$-values less than $\alpha$ has higher power.


\begin{figure}
  \centering
\includegraphics{toyExample-005}
\caption{\label{fig:toy-example-alpha-power} Proportion of randomizations that would reject the null hypothesis that $\theta = 0$ when $\theta = 1$ (``power'') of the two assignment methods (assigning 2 out of 6 or 3 out of 6 subjects to treatment) as a function of the $\alpha$-level employed. The top panel represent the case of the model of direct effects only, while the lower panel adds an indirect effect for any node that has at least one treated neighbor. The vertical gray line is at $\alpha = 0.10$}.
\end{figure}

Figure~\ref{fig:toy-example-alpha-power} compares the two assignment methods when spillover is and is not present with respect to power, as a function of the selected $\alpha$-level. As the figure shows, in the absence of spillover, the balanced design almost always possess better power characteristics than the unbalanced design. As power is a function of $p$-values generated for each randomization, it can be useful to consider the mean $p$-value of the sharp null hypotheses for these different methods, where lower mean $p$-values correspond to more power. Overall, for the balanced design the average $p$-value without spillover was $0.4$ while for the unbalanced design had mean $p$-values of $0.493$. Conversely, when spillover is present the unbalanced design generally has superior power to the balanced design, with an overall mean of  $0.547$ compared to $0.56$ for the balanced design. While the difference between the $p$-values for the spillover model is small, it is important to note that conventional wisdom holds that balanced designs always possess superior power advantages. When spillover is present, however, this is not universally true. In some situations, when spillover is present, unbalanced assignment can increase statistical efficiency.


